Differentially Private Synthetic Mixed-Type Data Generation For Unsupervised Learning

We introduce the DP-auto-GAN framework for synthetic data generation, which combines the low dimensional representation of autoencoders with the flexibility of Generative Adversarial Networks (GANs). This framework can be used to take in raw sensitive data and privately train a model for generating synthetic data that will satisfy similar statistical properties as the original data. This learned model can generate an arbitrary amount of synthetic data, which can then be freely shared due to the post-processing guarantee of differential privacy. Our framework is applicable to unlabeled mixed-type data, that may include binary, categorical, and real-valued data. We implement this framework on both binary data (MIMIC-III) and mixed-type data (ADULT), and compare its performance with existing private algorithms on metrics in unsupervised settings. We also introduce a new quantitative metric able to detect diversity, or lack thereof, of synthetic data.

==> intro-rel1-1.tex <==
Bayesian inference has also been used for differentially private data generation \citep{zhang2017privbayes,ping2017datasynthesizer} by assessing the correlation between features. We note the survey \cite{surendra2017review} on various techniques in private synthetic data generation upto 2016.

In 2016, \cite{abadi2016deep} introduces a framework for training deep learning models with differential privacy. Nonconvex optimization, required in training deep models, can be made differentially private by Gaussian mechanism: adding a Gaussian noise to a clipped (norm-bounded) gradient in each training step.  \cite{abadi2016deep}  introduces \textit{moment accountant} privacy analysis for private stochastic gradient descent in nonconvex optimization, which captures compositions of Gaussian mechanism more precisely than advanced composition \cite{DR14}. Moment account is later defined in terms of \textit{Renyi Differential Privacy (RDP)} \citep{mironov2017renyi}, which is a standard of privacy composition for differentially private stochastic gradient descent (DP-SGD). Due to success of training deep models with privacy guarantees, many previous works use deep (neural-network-based) generative models to generate synthetic data.   Those works can be broadly categorized into two types: autoencoder-based and GAN(Generative Adversarial Network)-based.


==> intro-rel1.tex <==
\subsection{Related Work}

\paragraph{Differentially Private Data Generation}
Existing works in differentially private synthetic data generation can be summarized in Table \ref{tab:data-gen}.

\begin{table}[t]
\caption{Previous algorithmic frameworks for differentially private synthetic data generation. Our algorithmic framework is the first to combine both DPGAN and autoencoder into one framework.}
\label{tab:data-gen}
\begin{center}
\begin{tabular}{|p{1.5cm}|p{2cm}|p{8.5cm}|}
\hline
\multirow{2}{*}{\bf \ \ \ \ Types}  &\multicolumn{2}{c|}{\bf Algorithmic framework} \\ \cline{2-3}
& \multicolumn{1}{c|}{\textbf{Main architecture}} & \multicolumn{1}{c|}{\textbf{Variants}}
\\ \hline
\multirow{7}{\linewidth}{Deep generative models}         &\multirow{4}{\linewidth}{DPGAN \cite{abadi2016deep} } & PATEGAN \cite{jordon2018pate} \\
& & DP Wasserstein GAN \cite{uclanesl_dp_wgan}\\
& & DP Conditional GAN \cite{torkzadehmahani2019dp} \\
& & Gumbel-softmax for categorical data \cite{frigerio2019differentially} \\ \cline{2-3}
& \multirow{3}{\linewidth}{Autoencoder}    & DP-VaE \cite{chen2018differentially,acs2018differentially} \\
& &                RBM generative models in latent space \cite{acs2018differentially} \\
& &                Mixture of Gaussian model in latent space \cite{abay2018privacy} 
\\ \hline

Other  models & \multicolumn{2}{p{10.5cm}|}{DataSynthesizer \cite{ping2017datasynthesizer}, PriBayes \citep{zhang2017privbayes} , SmallDB \cite{blr08}, PMW \citep{HR10}, among others}\\ \hline
\end{tabular}
\end{center}
\end{table}

[Rachel's part]

 small DP, PMW (anything else?),




==> intro-rel2.tex <==
\paragraph{Differentially Private Autoencoder-Based Generative Models} Variational autoencoder (VaE) \cite{kingma2013auto} is a generative model that compresses high-dimensional data to a smaller space called \textit{latent space}. The compression is commonly achieved through deep models and can be differentially private trained \citep{chen2018differentially,acs2018differentially}. VaE assumes that the \textit{latent distribution}, a distribution of data represented in latent space, is a Gaussian distribution; an assumption that is arguably unrealistic. \cite{acs2018differentially} uses Restricted Boltzmann machine (RBM) \cite{goodfellow2016deep} to learn the (unnecessarily Gaussian) latent distribution, and \cite{abay2018privacy} uses expectation maximization \cite{dempster1977maximum,park17EM} to learn mixture of Gaussian (instead of simple Gaussian). Our work extends this line of work by incorporating the generative model  GANs \citep{GAN14} which has shown success in synthesizing various types of data and distributions to learn latent distribution instead. The motivation is that GANs can more easily and efficiently learn distribution in compressed data-informative space than directly from unstructured, high-dimensional sparse data (e.g.  \cite{choi2017generating}.

\paragraph{Differentially Private GANs}
GAN is a generative model proposed by \citet{GAN14} with numerous follow-up works showing success for generating different types of data \citep{mogren2016c,saito2017temporal,salimans2016improved,jang2016categorical,kusner2016gans,wang2018graphgan}. 
As other deep models, GANs can be trained privately by aforementioned private stochastic gradient descent. We list the line of works that use private GANs for synthetic data generation.


Wasserstein GAN (WGAN) \citep{arjovsky2017wasserstein,Gulrajani17} is a variant of GANs obtained by using loss function motivated from Wasserstein distance in GAN training. The private WGAN are then implemented by
\cite{uclanesl_dp_wgan,triastcyn2018generating} among others.
Our work uses the GAN variant WGAN to define the loss objective.

Under the supervised setting (real data and data to be synthesized are with labels),  conditional GANs (CGAN) \citep{mirza2014conditional} train GANs under an auxiliary information, which can be a specific class of labels to generate datapoints of a label of choice.
Private version CGAN has been implemented by \cite{torkzadehmahani2019dp}. 
% \cite{triastcyn2018generating} proposes a framework that uses critics to obtain the label.
Private Aggregation of Teacher Ensembles (PATE) \citep{papernot2016semi,papernot2018scalable} are synthetic data generation framework proposed for semi-supervised setting of multi-label classification when some unlabelled public data are available. A variant of GAN called PATEGAN \citep{jordon2018pate} extends PATE to generate synthetic classification data when no public data is available.
 
There are numerous works on optimizing differentially private GANs (DPGANs). The performance of DPGANs can be improved by
data partitioning (either by class of labels in supervised setting or a private algorithm) \citep{yu2019differentially,papernot2016semi,papernot2018scalable,jordon2018pate,abay2018privacy,acs2018differentially,chen2018differentially}; 
reducing number of parameters in deep models \citep{mcmahan2017learning};
changing the clipping norm of gradient in DP-SGD during the training \citep{mcmahan2017learning,van2018three,thakkar2019differentially};
  changing noise of Gaussian mechanism over the training \citep{yu2019differentially}; 
and using public data of similar distribution to private one (if we have) to pre-train the model \citep{zhang2018differentially,mcmahan2017learning}.
  Clipping gradients per-layer of models \citep{mcmahan2018general,mcmahan2017learning} and per-dynamic parameter grouping \citep{zhang2018differentially} are also proposed.

Our work focuses on unsupervised setting -- data do not have any specific feature as label, or any public data of similar quality is available (however, unsupervised synthetic data generation like ours generalizes to supervised data by  treating a label as one feature). For fair comparison, we do not implement optimization techniques that were not present in previous works used as baseline. However, we include implementation details and discussions of optimizing DP-GANs in Appendix. 

Originally GANs are used to generate synthetic images. Later, architecture of DPGANs can be modified to generate other types of data such as categorical and time-series data \citep{frigerio2019differentially}. We now discuss deep generative models that can generate types of data beyond real-valued.



==> intro-rel3.tex <==
\paragraph{Data Generation for Different Types of Data}

%\textcolor{red}{[Note to Digvijay: this is where you can fill in]
%Note by Tao from the conversation that you (Digvijay can use) can use: this section should include the discussion on BOTH algorithmic and types of data the three papers generate: the two DP + autoencoder paper and then the LSTM (DP GAN + softmax) paper.
%Our story is as follow(s).\\
%- to both DP autoencoder paper: say that 1) we think \textit{data distribution in latent space is more complex} than a Gaussian (VAE) or mixture of Gaussian (so DP-EM was not performing well)
%2) they could have trained encoder without DP and DP just on decoder...\\
%- to the LSTM paper: our algorithm is very different. No autoencoder. Just one post processing of DP GAN via softmax layer to get categorical output.\\
%We should also mention that "very wrong" paper somewhere - maybe here and 5 reasons why it's bad.} \\
Here we discuss recent works that can generate differentially private synthetic data of mixed type.% i.e., dataset in which some features are real valued and some are discrete valued.
\citet{abay2018privacy} considers the problem of generating mixed type labeled data where number of labels is $k$. Their algorithm, DP-SYN, partitions the dataset into $k$ sets based on the labels and on each partition, trains a DP auto-encoder. Then a DP expectation maximization (DP-EM) algorithm by \citet{park17EM} is used to learn the distribution in the latent space of encoded data of the given label-class. %A new sample of data generated from DP-EM is fed to the  decoder of the DP auto-encoder. This process is repeated for all $k$ label-classes to obtain a DP synthetic dataset. 
The main workhorse, DM-EM algorithm, is designed and analyzed for mixture of Gaussian model and more general factor analysis model \citep{park17EM}.

\citet{chen2018differentially} works in the similar setting as before. In particular, they used differentially private variational auto-encoder (DP-VaeGM) to generate mixed type labeled data with $k$ labels. DP-VaeGM trains a DP variational auto-encoders (DP-Vae) on each of the $k$ partitions. %Synthetic data for a given class is generated using Gaussian samples and differentially private Vae model of that class. 
This algorithm replaces the combination of DP auto-encoder and DP-EM in \citet{abay2018privacy} by DP-Vae. DP-VaeGM assumes that the posterior, i.e., mapping from real data to Gaussian, can be efficiently learned using encoder neural network.

\citet{frigerio2019differentially} used WGAN to generate differentially private mixed type synthetic data. The algorithmic framework is to use WGAN with DP-SGD algorithm to obtain DP WGAN which is similar to the one proposed in \citet{zhang2018differentially,xie2018differentially}who focused on image datasets. Methodology of \citet{frigerio2019differentially} for generating mixed synthetic data involves two main ingredients: change of discrete data to binary data using one-hot encoding and a tweak the architecture of the generator in WGAN by adding an output softmax layer for every discrete variable.

Our framework is distinct from all of the relevant DP frameworks mentioned above. We use a differentially private auto-encoder which, unlike Vae \citep{chen2018differentially}, does not require the necessity of mapping to a Gaussian distribution. This also allows us to reduce the dimension of the problem to be handled by WGAN hence escaping the issues of high-dimensionality due to one-hot encoding of \citet{frigerio2019differentially}. We also use DP-GAN, replacing DP-EM in \citet{abay2018privacy}, for learning distribution in the latent encoded space. Now we review the evaluation schemes for measuring quality of synthetic data.
\paragraph{Evaluation Metric of Synthetic Data}
%\textcolor{red}{
%[Tao's note: I think it is good to put the motivation of why we pick MIMIC 3 and UCLA data as baseline here]\\
%- why pick MIMIC3? Because of the connection we build on MedGAN.\\
%- Then we claim that this MedGAN architecture can be made DP and then for \textit{any} type of data, not just all binary\\
%- So we go search for papers that does mixed types. Only 2 DP autoencoders paper and LSTM paper (e.g. on Adult dataset from Census 1994), but they all use supervised learning metric. Data generation we want to focus is unsupervised.\\
%- So we adapt the Census NIST2018 challenge one (the other one with mixed-type) because the metric designed in the challenge is unsupervised in nature. So we pick the UCLA WGAN algorithm to compare.}

Various evaluation metrics have been considered in the literature to quantify the quality of the synthetic data \citep{charest2011can}. Broadly, evaluation metrics can be divided into two major categories: supervised  and unsupervised.

\textit{Supervised evaluation metrics}: These metrics are used when clear distinctions exist between feature and labels of the dataset, e.g., for healthcare applications, whether a person has a disease or not could be a label. The main aim of generating synthetic data is to best understand the relationship between features and labels. A popular metric for such cases is to train a machine learning model on the synthetic data and report its accuracy on the real test data\citep{xie2018differentially}. \citet{zhang2018differentially} used inception scores on the image data with classification tasks. Inception scores were proposed in \citet{salimans2016improved} for images which measure quality as well as diversity of the generated samples. Another metric used in \citet{jordon2018pate} reports whether the accuracy ranking of different machine learning models trained on the real data is preserved when the same machine learning model is trained on the synthetic data. All the evaluation metrics focus on understanding relationship between labels and features of the data and hence we call them supervised evaluation metrics. Also, in the literature, these metrics are used for classification setting but can be generalized to regression setting easily.
\begin{table}[h]
	\caption{Summary of  evaluation metrics in DP synthetic data generation. We list applicability of each metric to each of the data type. Evaluation methods with asterisk * indicates that the methods are specified by a predictive model of choice, and their applicability therefore depends on types of data such predictive model is appropriate for. Our neural-based metric adds another choice of model to dimension-wise prediction in an unsupervised setting}
	\label{tab:metric}
	\begin{center}
		\begin{tabular}{lp{4cm}p{2cm}p{2cm}p{2.5cm}}
			\multicolumn{1}{c}{\bf SETTINGS}  &\multicolumn{1}{c}{\bf EVALUATION METHODS}  & \multicolumn{3}{c}{\bf DATA\ TYPES} \\
			\multicolumn{1}{c}{\bf }  &\multicolumn{1}{c}{\bf } & \multicolumn{1}{c}{\bf Binary} & \multicolumn{1}{c}{\bf Categorical} & \multicolumn{1}{c}{\bf Regression}
			\\ \hline \\
			\multirow{2}{*}{Supervised}         & Label prediction* \citep{chen2018differentially,abay2018privacy, frigerio2019differentially} & Yes & Yes & Yes\\
			&Predictive model ranking* \citep{jordon2018pate} & Yes & Yes & Yes \\ \hline
			\multirow{3}{*}{Unsupervised} 
			&Dimension-wise probability plot \citep{choi2017generating} & Yes & No & No \\
			&Dimension-wise prediction plot* & Yes (\cite{choi2017generating} and ours) & Yes (ours) & Yes (ours) \\
			&\(k\)-way marginal  \cite{NIST2018Match3} & Yes & Yes  & Yes  \\
		\end{tabular}
	\end{center}
\end{table}

\textit{Unsupervised evaluation metric}: These metrics are used when no feature of the data can be decisively termed as a label. \citet{zhang2018differentially} also provides a Jensen-Shannon score metric which measures the Jensen-Shannon divergence between output of a discriminating neural network on the real and synthetic dataset, and a Bernoulli random variable with $0.5$ probability. Dimension-wise probability is a popular measure proposed in \citet{choi2017generating} for binary data. It compares the marginal distribution of real and synthetic data on each individual feature. Dimension-wise prediction is another measure that measures how closely synthetic data captures inter-feature relationships in the real data. This was proposed for binary data and we extend this to mixed type data. Recently, \citet{NIST2018Match3} challenge used a 3-way marginal evaluation metric in which random three feature of the real and synthetic data are used to compute the total variation distance as a statistical score. This process is repeated a few times and finally, average score is returned. Table \ref{tab:metric} provides an overview of these metrics.

==> metric.tex <==
\section{Evaluation Metrics}\label{s.metric}

%Overall pictures of metric we will use:
%
%\begin{enumerate}
%\item MedGAN (3 metrics): dim-wise prob; dim-wise F1 score on feature with at least 1 percent diversity; AUC score. (all three for baseline comparison to DP paper
%\item Census (2 metrics):  marginal (for fair comparison to NIST); NNs dim-wise prediction (generalization of MedGAN metric from all-binary data to mixed-type data)
%\end{enumerate}
%
%[Digvijay]: discuss each of the metric we use in overview (e.g. motivation) in words, and also in mathematically precise form.
%

%\rc{this paragraph can be moved to somewhere in section 3 if it fits better there, once that section is all written}
%The DP-auto-GAN framework described in Section \ref{s.algo} can be used to take in raw sensitive data, and privately train a model for generating synthetic data that should satisfy the same statistical properties as the original data.  This learned model can be used to generate arbitrary amounts of publicly available synthetic data, which can then be freely shared due to the post-processing guarantees of differential privacy.

%Since the DP-auto-GAN algorithm is differentially private, than any data generated in this way will also be differentially private with respect to the original data, by the post-processing guarantees of differential privacy.

%In Section \ref{s.exp}, we implement the DP-auto-GAN framework to empirically validate its performance on two different datasets: the \mimic dataset \cite{uci_ml}, which has only binary features, and the ADULT dataset \cite{uci_ml}, which has binary, categorical, and real-valued features.  
In this section, we discuss the evaluation metrics that we use in the experiments (described in Section \ref{s.exp}) to empirically measure the quality of the synthetic data. Some of these metrics have been used in the literature, while many are novel contributions in this work. The evaluation metrics are summarized  in Table \ref{tab:metric}; our contributions are in bold.  

\begin{table}[h]
        \caption{Summary of  evaluation metrics in DP synthetic data generation. We list applicability of each metric to each of the data type. Parts in \textbf{bold} are \textbf{our new contributions}. Evaluation methods with asterisk * are predictive-model-specific, and their applicability therefore depends on types of data that the chosen predictive model is appropriate for. 
Methods with asterisks ** are equipped with any any distributional distance of choice such as Wasserstein distance.  
%Our neural-based metric adds another choice of model to dimension-wise prediction in an unsupervised setting
}
        \label{tab:metric}
        \begin{center}
                \begin{tabular}{p{2.6cm}p{5.3cm}p{1.5cm}p{1.5cm}p{1.5cm}}
                        \bf {TYPES}
&\multicolumn{1}{c}{\bf EVALUATION METHODS}  & \multicolumn{3}{c}{\bf DATA\ TYPES} \\
                        \multicolumn{1}{c}{\bf }  &\multicolumn{1}{c}{\bf } & \multicolumn{1}{c}{\bf Binary} & \multicolumn{1}{c}{\bf Categorical} & \multicolumn{1}{c}{\bf Regression}
                        \\ \hline \\
                        \multirow{2}{*}{Supervised}         & Label prediction* \citep{chen2018differentially,abay2018privacy, frigerio2019differentially} & Yes & Yes & Yes\\
                        &Predictive model ranking* \citep{jordon2018pate} & Yes & Yes & Yes \\ \hline
                        \multirow{1}{\linewidth}{Unsupervised, prediction-based } 
                        &Dimension-wise prediction plot* & Yes (\cite{choi2017generating}, \textbf{ours}) & \textbf{Yes} & \textbf{Yes} \\ \hline
\multirow{4}{\linewidth}{Unsupervised, distributional-distance-based } 
                        &Dimension-wise probability plot \citep{choi2017generating} & Yes & No & No \\
                        &\(3\)-way feature marginal, total variation distance \citep{NIST2018Match3} & Yes & Yes  & Yes  \\
                        &\textbf{\(k\)-way feature marginal**}  & \textbf{Yes} & \textbf{Yes} 
& \textbf{Yes} 
\\
                        &\textbf{\(k\)-way PCA marginal**} & \textbf{Yes} & \textbf{Yes}  & \textbf{Yes}  \\
                        &\textbf{Distributional distance**} & \textbf{Yes} & \textbf{Yes}  & \textbf{Yes}  \\ \hline
\multirow{2}{\linewidth}{\textbf{Unsupervised, qualitative}} 
                        &\textbf{\(1\)-way feature marginal (histogram)}& \textbf{Yes} & \textbf{Yes}  & \textbf{Yes}  \\
                        &\textbf{\(2\)-way PCA marginal (data visualization)} 
& \textbf{Yes} & \textbf{Yes}  & \textbf{Yes}  \\
                \end{tabular}
        \end{center}
\end{table}

For the first two metrics described below, the dataset should be partitioned into a training set $R \in \Rbb^{m_1 \times n}$ and testing set $T \in \Rbb^{m_2 \times n}$, where $m = m_1+m_2$ is the total number of samples the real data, and $n$ is the number of features in the data. After training the DP-auto-GAN, we use it to create a synthetic dataset $S \in \Rbb^{m_3\times n}$, for sufficiently large $m_3$.



%First, we used \mimic dataset. This dataset is used since we build our DP-GAN based on medGAN architecture proposed in \cite{choi2017generating} which used \mimic dataset to showcase the usefulness of medGAN. \cite{xie2018differentially} also used this dataset in their experiments on generating DP synthetic data using GANs. Note that this is a binary dataset for which metrics are already proposed in the literature as follows.

%In this case, we divide \mimic dataset into a training set $R \in \{0,1\}^{m_1 \times n}$ and testing set $T \in \{0,1\}^{m_2 \times n}$in ratio $4:1$. Here $n$ is the dimension of the data and $m = m_1+m_2$ is the total number of samples the real data. We also create a synthetic dataset $S \in \{0,1\}^{m_3\times n}$ for sufficiently large value of $m_3$. Then we have the following metrics:

\textbf{Dimension-wise probability.} This metric is used when the entire dataset is binary, and it serves as a basic sanity check to verify whether \dpgan has correctly learned the marginal distribution of each feature. Specifically, it compares the proportion of $1$'s (which can be thought of as estimators of Bernoulli success probability) in each feature of the training set $R$ and synthetic dataset $S$.%In particular, we compare the proportion of $1$'s (which can be thought of as estimators of Bernoulli success probability) in each feature of training set $R$ and synthetic dataset $S$. 

\textbf{Dimension-wise prediction.} This metric evaluates whether \dpgan has correctly learned the relationships \emph{between} features. For the $k$-th feature of training set $R$ and synthetic dataset $S$, we choose $y_{R_k} \in \Rbb^{m_1}$ and $y_{S_k} \in \Rbb^{m_3}$ as labels of a classification or regression task based on the type of that feature, and the remaining features $R_{-k}$ and $S_{-k}$ are used for prediction. We train either a classification or regression model and measure goodness of fit based on the model's accuracy using the following well known metrics: 
\begin{enumerate}
\item Area under the ROC curve (AUROC) score and $F_1$ score for classification: The $F_1$ score of a classifier is defined as
$F_1 := \tfrac{2\times \text{precision} \times \text{recall}}{\text{precision} + \text{recall}},$
where precision is ratio of true positives to true and false positives, and recall is ratio of true positives to total true positives (i.e., true positives plus false negatives). AUROC score is a graphical measure capturing the area under ROC (receiver operating characteristic) curve, and is only intended for binary data.  Both metrics take values in interval $[0,1]$ with larger values implying good fit. 
\item $R^2$ score for regression: The $R^2$ score is defined as
$1 - \tfrac{\textstyle{\sum} (y_i-\wh{y}_i)^2}{\textstyle{\sum} (y_i - \wb{y})^2} ,$
where $y_i$ is the true label, $\wh{y}_i$ is the predicted label, and $\wb{y}$ is the mean of the true labels. This is a popular metric used to measure goodness of fit as well as future prediction accuracy for regression.
\end{enumerate}


% using the following well known metrics: \\
% 1. Area under the ROC curve (AUROC) score and $F_1$ score for classification: The $F_1$ score of a classifier is defined as
% $F_1 := \tfrac{2\times \text{precision} \times \text{recall}}{\text{precision} + \text{recall}},$
% where precision is ratio of true positives to true and false positives, and recall is ratio of true positives to total positives. AUROC score is graphical measure capturing area under ROC (receiver operating characteristic) curve. Both metrics take values in interval $[0,1]$ with larger values implying good fit. \\
% 2. $R^2$ score for regression: $R^2$ score is defined as
% $1 - \tfrac{\textstyle{\sum} (y_i-\wh{y}_i)^2}{\textstyle{\sum} (y_i - \wb{y})^2} ,$
% where $y_i$ is the true label, $\wh{y}_i$ is the predicted label and $\wb{y}$ is the mean of the true labels. This is a popular metric used to measure goodness of fit as well as future prediction accuracy for regression.


%\rc{Which of these metrics have been used before, and which ones are we claiming as our contributions? Are all the binary ones prior and all the mixed-type ours? Or only some of the mixed type?}

%In this section, we provide details of the evaluation metrics we used to empirically validate the quality of synthetic data generated. 

%Our DP-auto-GAN framework can handle mixed-type data. However, we first evaluate it on \mimic dataset, which is a completely binary dataset. We use this dataset in order to have a fair comparison with existing works in the literature \citep{choi2017generating,xie2018differentially}.
We also propose following novel evaluation metrics. 

\textbf{1-way feature marginal.} This metric works as a sanity check for real features. We compute histograms for the feature interest of both real and synthetic data. The quality of  the synthetic data with respect to this metric can be evaluated qualitatively through visual comparison of the histograms on real and synthetic data.  This can be extended to $k$-way feature marginals and made into a quantitative measure by adding a distance measure between the histograms.

\textbf{2-way PCA marginal.} This metric generalizes the 3-way marginal score used in \citet{NIST2018Match3}. In particular, we compute principle components of the original data and evaluate a projection operator for first two principle components. Let us denote $P\in \Rbb^{n\times 2}$ as the projection matrix such that $\wb{R} = RP$ is the projection on first two principle components of $R$. Then we evaluate projection of synthetic data $\wb{S} = SP$ and scatterplot 2-D points in $\wb{R}$ and $\wb{S}$ for visual evaluation. For quantitative evaluation, we also compute Wasserstein distance between $\wb{R}$ and $\wb{S}$. In the simulations described in Section \ref{s.exp}, we used Wasserstein distance since we optimize for the WGAN objective, but any distributional divergence metric can be used. This approach can also be extended to $k$-way marginals by making the projection matrix $P\in \Rbb^{n\times 2}$ for the first $k$ principle components.

\textbf{Distributional distance.} In this metric, we first compute the Wasserstein distance  \(W_2(R,S)\) between the entire real and synthetic datasets \(R,S\). The Wasserstein score is then defined as
\begin{equation*}
W_\text{score}(R,S):=1-\tfrac{W_2(R,S)}{\max_{x,y\in \XX} ||x-y||_2^2},
\end{equation*} 
%\rc{add more here. There's a lot of metrics listed in the table}
where the Wasserstein distance is normalized by the maximum distance possible of two datapoints in data universe $\XX$. To compute the Wasserstein score on \(k\)-way marginal PCA projection \(P\), we normalize  the score  with additional term \(\sqrt{v}\), where \(v\) is the explained variance of \(P\):
\begin{equation*}
W_\text{score}(\bar R,\bar S,P):=1-\tfrac{W_2(\bar R,\bar S)}{\sqrt{v}\max_{x,y\in \XX} ||x-y||_2^2}.
\end{equation*}


 For more details about implementation of these new evaluation metrics, their generalizations and relationships among them, we refer the reader to Appendix \ref{app.met}.


==> prelim-DP.tex <==
\section{Preliminary} \label{prelim}
\subsection{Differential Privacy (DP)} \label{sec:DP}
[Rachel's part]

